An Exploratory Study on Regression Vulnerabilities

Background: Security regressions are vulnerabilities introduced in a previously unaffected software system. They often happen as a result of source code changes (e.g., a bug fix) and can have severe effects. Aims: To increase the understanding of security regressions. This is an important step in developing secure software engineering. Method: We perform an exploratory, mixed-method case study of Mozilla. First, we analyze 78 regression vulnerabilities and 72 bug reports where a bug fix introduced a regression vulnerability at Mozilla. We investigate how developers interact in these bug reports, how they perform the changes, and under what conditions they introduce regression vulnerabilities. Second, we conduct five semi-structured interviews with as many Mozilla developers involved in the vulnerability-inducing bug fixes. Results: Software security is not discussed during bug fixes. Developers' main concerns are the complexity of the bug at hand and the community pressure to fix it. Moreover, developers do not to worry about regression vulnerabilities and assume tools will detect them. Indeed, dynamic analysis tools helped finding around 30% of regression vulnerabilities at Mozilla. Conclusions: These results provide evidence that, although tool support helps identify regression vulnerabilities, it may not be enough to ensure security during bug fixes. Furthermore, our results call for further work on the security tooling support and how to integrate them during bug fixes. Data and materials: https://doi.org/10.5281/zenodo.6792317

==> tables/SPK_Description.tex <==
\begin{table}[htbp]
  \centering
    \begin{tabular}{|p{10em}|p{15em}|}
    \hline
    \multicolumn{1}{|c|}{\textbf{Categories}} & \textbf{Description} \\
    \hline
    Input Validation \& Representation (IVR) & Security problems resulting from trusting input. (Buffer Overflow, Cross-site scripting, Unsafe Reflection, Integer Overflow, etc.) \\
    \hline
    API Abuse (AA) & Violation of a caller-callee contract \\
    \hline
    Security Features (SF) & Problem related to authentication, access control, confidentiality, cryptography, privilege management, etc. \\
    \hline
    Time and State (TS) & Defects related to unexpected interactions between threads, processes, time, and information. \\
    \hline
    Error Handling (Err) & Rough or no handling of errors and exceptional conditions, exposing too much information through error handling. \\
    \hline
    Indicator of Poorly Written Code (IPWC) & Poorly written code leading to unexpected behavior. \\
    \hline
    Encapsulation (Enc) & Unspecified or weak boundaries, lack of trust or trust models \\
    \hline
    \end{tabular}%
    \caption{An Overview of Seven Pernicious Kingdom Taxonomy.}%
  \label{tab:SPKdescription}%
\end{table}%


==> tables/incorrect_fix_types.tex <==
\begin{table}[]
  \centering
  \caption{Classification of incorrect fixes and security regressions.}
    \begin{tabular}{lrr}
    \toprule
    \textbf{Types} & \multicolumn{1}{l}{\textbf{incorrect Fixes }} & \multicolumn{1}{l}{\textbf{Security Regressions}} \\
          & \multicolumn{1}{c}{Total=36} & \multicolumn{1}{c}{Total=36} \\
    \midrule
    Check & 1     & 2 \\
    Timing & 0     & 4 \\
    Logic & 2     & 2 \\
    Resource & 7     & 28 \\
    Structural & 15    & 0 \\
    Large defects & 11    & 0 \\
    \midrule
    \textbf{Large or Complex fixes} & 28    & 8 \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> tables/tab-interview-questions.tex <==
%!TeX root = ../esem22-regressions.tex

\begin{table} [b]
	\centering 
	\caption{Sample of the interviews questions.} 
	\label{tab:interview-questions}
	\begin{tabular}{ll}
		\hline
		Q2 & Could you please explain what regressions are? \\ 
		Q7 & What do you or your team does to avoid introdu- \\
		      &  cing regression vulnerabilities during bug fixes?  \\ 
		\hline
	\end{tabular}
\end{table}
